Towards providing reliable job completion time predictions using PCS

In this paper we build a case for providing job completion time predictions to cloud users, similar to the delivery date of a package or arrival time of a booked ride. Our analysis reveals that providing predictability can come at the expense of performance and fairness. Existing cloud scheduling systems optimize for extreme points in the trade-off space, making them either extremely unpredictable or impractical. To address this challenge, we present PCS, a new scheduling framework that aims to provide predictability while balancing other traditional objectives. The key idea behind PCS is to use Weighted-Fair-Queueing (WFQ) and find a suitable configuration of different WFQ parameters (e.g., class weights) that meets specific goals for predictability. It uses a simulation-aided search strategy, to efficiently discover WFQ configurations that lie on the Pareto front of the trade-off space between these objectives. We implement and evaluate PCS in the context of DNN job scheduling on GPUs. Our evaluation, on a small scale GPU testbed and larger-scale simulations, shows that PCS can provide accurate completion time estimates while marginally compromising on performance and fairness.

==> rest.tex <==
\section{Other Related Work}
\label{sec:related work}

\paragraph{DNNs under resource constraints.}
A large body of work has looked at the problem of compressing trained DNN models to optimize their pipeline for faster inference and lower resource consumption~\cite{modular-dnn, chameleon, noscope, mcdnn}.
MCDNN (\cite{mcdnn}) uses a trained DNN model to create different variants with varying accuracy and resource usage.
NoScope (\cite{noscope}) compresses complex DNNs trained for face detection to specialized models that compromise on generality for much faster inference.
Chameleon (\cite{chameleon}) dynamically picks the best configuration from an array of pre-trained DNN based video analytics pipelines based on available computational resources.
Efforts like reference \cite{modular-dnn} construct DNNs so they can be partially downloaded.
% by clients. in case network bandwidth is limited.
Our vision of resource adaptive DNNs shares some techniques utilized by these proposals, for example resource based architectural modifications, but there are important differences as well.
For instance, most of these strategies focus on optimizing inference, which is a less dynamic problem than optimizing a DNN \emph{during} training.


\begin{comment}
\paragraph{Network aware applications.}
The idea of adapting applications to network conditions has been used for a variety of applications.
Video bitrate adaptation (\cite{pensieve}) techniques lower the quality of video frames based on available bandwidth.
AWStream (\cite{awstream}) presents resource aware stream processing operators which provide graceful degradation if network bandwidth is low.
Adapting query executions based on network conditions has also been shown to improve performance (\cite{optimize-query}).
These proposals show that application level adaptation is beneficial, independent of how network resources are managed.
\end{comment}


\begin{comment}
\paragraph{Richer Interfaces in Other Contexts.} Application adaptation to degraded network conditions has been looked at extensively in the context of mobile systems. 
Availability of the network and its varying bandwidth is a big concern for mobile clients. Systems like ~\cite{odyssey,multi-fidelity} modify behavior of client software running on mobile devices based on bandwidth estimation, CPU usage and battery power consumption. 
However, the middleware used by these systems (and its interface) is specifically tailored for the needs of the mobile application, and
considers a best-effort network with no smarts.  

%cannot make use of technological trends in the network data plane.

Recently, MittOS~\cite{mittos} uses a richer interface between applications
and the storage stack to provide improved performance guarantees. The interface specifies a desired latency requirement -- the storage
stack rejects the request if the latency cannot be provided. 
Our proposal is similar in spirit, but focuses on the unique challenges of the network resource, 
and also considers richer applications, which can adapt in different ways based on the network feedback. 
These differences require a richer API than the one used in MittOS. 
\end{comment}

%fast IO rejection %method for storage systems for requests with deadlines. It predicts whether an IO will meet its deadlines based on the backlog at the disk scheduler.


%\paragraph{Guarantees in the cloud.} Works like Cicada ~\cite{cicada} and Mittos ~\cite{mittos} take on the challenge of providing resource guarantees to tenants in the cloud. These efforts are orthogonal to our vision of a talkative network which indeed relies on predictability %and guarantees at the network layer that these ideas may have to offer. Cicada monitors network resource usage on behalf of tenants and uses them to predict data rate requirements at a future interval, using these to provide bandwidth guarantees. Mittos uses a fast IO rejection %method for storage systems for requests with deadlines. It predicts whether an IO will meet its deadlines based on the backlog at the disk scheduler.


% Efforts like Clipper~\cite{clipper} minimize inference latency of deployed machine learning models by combining the results of several models together
\paragraph{Inference systems.} The networking community has realized the importance of machine learning applications.
Recent systems like Clipper~\cite{clipper} minimize inference latency of deployed machine learning models by combining the results of several models together,
while Ray~\cite{ray} is a high performing distributed framework for training reinforcement learning models for emerging AI applications.
 



% \sys{} is inspired by decades of research on new network architectures, such as DTN~\cite{dtn}, CCN~\cite{Jacobson09}, indirection-based architectures~\cite{i3}, and pub/sub systems~\cite{pubsub, pursuit}. A fundamental difference arises because of slack: if the network is connected, all these prior systems will \emph{immediately} deliver the data while \sys{} may not. 
% Thus, slack leads to different design choices. For example, \sys{} uses both push and pull modes while existing systems either use a push mode (e.g., DTN~\cite{dtn}, pub/sub~\cite{pursuit}) or a pull mode (e.g., CCN), but not both. Similarly, while DTN and CCN make use of in-network storage, \sys{} uses it in a novel way: in-network storage can be addressed (using MIDs) and services can be added on-the-fly while data is in transit. Unlike other indirection based architectures (e.g., i3~\cite{i3}), \sys{} has an explicit notion of in-network storage, so data can stay inside the network for arbitrary amount of time. 

%\sys{} also uses building blocks, such as hop-by-hop transport~\cite{hop09, tapaconext}, and self-certifying addresses (e.g., %AIP~\cite{aip-sigcomm2008}, XIA~\cite{xiansdi}). The benefits of these mechanisms are well-known; \sys{} uses them to support %slack-aware networking. 


%\paragraph{Routing.} While the routing problem is well-studied in the context of the Internet, the focus is on  finding a suitable %path which meets the QoS objectives of the application. In our case, the addition of slack adds the timing dimension (i.e, scheduling) %to the traditional routing problem because we need to not only decide which path to use but also how long each node will store the %ADU. In this way, the problem is similar to the routing problem in delay tolerant networks, although the constraints and objectives %are different. We have a connected network with slack and cost consideration while DTN routing typically focuses on minimizing %end-to-end delay under intermittent connectivity. 
%Our work is most similar to NetStitcher which also consider the joint routing and scheduling problem for bulk data transfer between %datacenters. However, it does not consider typical cloud pricing models that result in different costs for using different paths %depending on the time. 
%The consideration of cost makes the problem challenging, both in terms of modelling and finding optimal solution in polynomial time. 
%Recently, X et al. consider bidding strategies for using the cloud, but their focus is only on compute research inside a single data %center which results in a single price whereas we consider multiple data centers (nodes) which may have different usage costs %depending on their respective peak hours. 



\section{Conclusion}
In this paper, we present our vision of resource adaptive DNNs and show its feasibility as well as the key challenges involved in realizing this vision. 
We believe that as DNNs gain more traction, making them adaptive -- for improved efficiency and performance -- will become even more important. The research agenda we present is rich and requires efforts from both the ML and systems communities. 


%However, to realize adaptive DNNs, we need to solve four important challenges:  (1) how to adapt DNNs %automatically?, (2) how to amortize the performance penalty of dynamically changing the DNN?, (3) how to obtain %resource information from the underlying system through a suitable interface?, and (4) how to use suitable %resource management policies at the bottom that are amenable to  resource adaptive DNNs at the top?
%We borrow (and extend) techniques from the ML (e.g., transfer learning, NAS, etc) as well as the networking %community (e.g., intelligent scheduling) to address these challenges.

\begin{comment}
\section{Discussion and Summary}
\label{sec:discussion}
\paragraph{Resource aware infrastructure.} 
For the emerging complex cyber-physical systems, we see the network as only one part of the overall resource usage footprint of these demanding applications. 
These systems make extensive use of specialized hardware, such as accelerated Graphical Processing Units (GPUs) and Tensor Processing Units (TPUs), which also currently support narrow interfaces. 
We envision the possibility of creating a comprehensive resource aware infrastructure, where every potential bottleneck resource can implement ``talkative'' interface, providing hints (such as GPU task queue length) to the applications, 
allowing them to modulate their behavior accordingly.

%\paragraph{Reward system for elastic applications.}
%We have seen the virtue of applications collaborating with a potentially congested network to achieve a common goal: maximizing utility while meeting latency and deadline constrains. Given the elastic nature of many cloud applications, is there an incentive for applications to %\emph{willingly} give up some of their share of network resources as long as the compromise on quality is bounded?  We believe that application elasticity can potentially be factored into the cloud pricing models to provide rewards (resource credits, lower prices) to such generous %applications.

\paragraph{Other applications.}
%While our focus is on next generation applications, we consider how existing applications can benefit from a talkative network.
%Augmented Reality (AR) is commonly used for coordinated tasks where multiples users are simultaneously manipulating a virtualised environment (classroom, map).
%Frequent network outages in such learning environments can frustrate the user and make the coordinating task an unpleasant experience. If such applications are proactively informed about the deteriorating network conditions they can employ auditory and visual notifications for the %users, communicating or masking network degradation.
The concept of talkative networks is potentially useful for a broad range of applications. Some applications have inherent elasticity in form of delay tolerance ~\cite{dtn}. They can delay sending traffic if the network informs them about its potentially congested state.
Similarly, responses for search applications have concave quality profiles ~\cite{zeta} -- given more time the result can be further improved. Applications can smartly choose the time budget for searching through indexes etc. based on the network latency budget.

\paragraph{Summary.} Our work is the first to look at systematically exploiting elasticity in emerging applications based on network feedback. We have discussed the research possibilities that such an approach opens up, gearing application design to judiciously exploit network awareness and designing network level mechanisms that are able to provide guarantees and accurate estimates to the application. The crucial bit is the interface that allows the the application and the network to work together. To this end, we provide a simple yet extensible API that we hope acts as a catalyst for future research in realizing our vision of talkative networks.
\end{comment}


%\paragraph{Impact on Developing Regions.}
%In such settings, users have different tolerance for delay (or slack), and 
%performance, cost, and privacy concerns can be much different from what we consider in the context of developed countries~\cite{}. 
%We believe that \sys{} can potentially have broader applicability in such environments where it can be used 
%for human-centric applications (e.g., web), in addition to the applications we discussed in this paper.
%These environments would present different trade-offs which may also lead to different choices of protocols for the hop-by-hop %transport and slack-aware routing than the ones discussed in the paper. 


% \paragraph{Summary.} In this paper, we make a case for slack-aware networking for a machine-centric future Internet. 
% To highlight the opportunities and challenges, we present \sys{}, which exposes slack information to multiple levels of the stack and uses decoupling of sender and receiver through in-network storage. \sys{} offers interesting opportunities at all levels of the stack, including the interface, transport services, and routing and forwarding. We hope this paper will act as a catalyst for a more concerted effort towards understanding the challenges and opportunities that arise in the emerging machine centric Internet. 


%In such environments, the 
%In such regions, the peculiar characteristics of the network connectivity, combined with slack information, may lead to innovative %solutions at different layers. For example, 






==> tables/table-intro.tex <==
\begin{table}[]
\begin{tabular}{@{}ccccc@{}}
\toprule
 & \begin{tabular}[c]{@{}c@{}}Avg\\ JCT\end{tabular} & \begin{tabular}[c]{@{}c@{}}Max\\ Unfairness\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg\\ \ecte{}\end{tabular} & \begin{tabular}[c]{@{}c@{}}p99 \\ \ecte{}\end{tabular} \\ \midrule
Tiresias & \textbf{35 hrs} & 95\% & 21\% & 340\% \\
Themis & 70 hrs & \textbf{18\%} & 24\% & 167\% \\
YARN-FIFO & 180 hrs & \textgreater{}500\% & \textbf{0\%} & \textbf{0\%} \\ \bottomrule
\end{tabular}
    \caption{Tiresias~\cite{tiresias} which optimizes for avg JCTs, Themis~\cite{themis} which aims to minimize unfairness and YARN-FIFO~\cite{YARN} for workload-2~(\S\ref{sec:eval}) on a simulated 64 GPU cluster.
    % Unfairness is defined as $max(0,\frac{JCT}{JCT_{fair}}-1)$ where $JCT_{fair}$ is the fair-finish time.
    For all metrics, lower is better.
    Preemptive scheduling strategies achieve optimal performance or fairness but are not predictable.}
    \label{table:trade-off-space}
\end{table}

==> tables/table-micro-eval-time.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lllllll@{}}
\toprule
Jobs  & 32       & 64       & 128      & 256      & 512     & 1024    \\ \midrule
512  & 5$\pm$2     & 5$\pm$2     & 6$\pm$2     & 5$\pm$2     & 4$\pm$1    & 7$\pm$3    \\
1024 & 43$\pm$26   & 51$\pm$31   & 54$\pm$29   & 50$\pm$30   & 35$\pm$22  & 31$\pm$4   \\
2048 & 168$\pm$107 & 246$\pm$133 & 249$\pm$142 & 206$\pm$134 & 159$\pm$97 & 150$\pm$60 \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/table-traces-jct.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
\begin{tabular}[c]{@{}c@{}}Scheduling\\ Policy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Trace \\ 0e4a51\end{tabular} & \begin{tabular}[c]{@{}c@{}}Trace \\ b436b2\end{tabular} & \begin{tabular}[c]{@{}c@{}}Trace \\ 6214e9\end{tabular} & \begin{tabular}[c]{@{}c@{}}Trace \\ 6c71a0\end{tabular} & \begin{tabular}[c]{@{}c@{}}Trace \\ 2869ce\end{tabular} & \begin{tabular}[c]{@{}c@{}}Trace \\ 7f04ca\end{tabular} & \begin{tabular}[c]{@{}c@{}}Trace \\ ee9e8c\end{tabular} \\ \midrule
AFS & \begin{tabular}[c]{@{}c@{}}avg JCT: 1.0\\ p99 JCT: 1.5\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.0\\ 1.0\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.0\\ 1.0\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.0\\ 1.0\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.0\\ 1.0\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.0\\ 1.0\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.0\\ 1.0\end{tabular} \\
SRSF & \begin{tabular}[c]{@{}c@{}}avg JCT: 1.1\\ p99 JCT: 2.0\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.3\\ 1.3\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.1\\ 1.2\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.1\\ 1.2\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.4\\ 2.6\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.1\\ 1.2\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.6\\ 1.5\end{tabular} \\
FIFO & \begin{tabular}[c]{@{}c@{}}avg JCT: 9.3\\ p99 JCT: 1.7\end{tabular} & \begin{tabular}[c]{@{}c@{}}60.0\\ 2.2\end{tabular} & \begin{tabular}[c]{@{}c@{}}92.0\\ 5.2\end{tabular} & \begin{tabular}[c]{@{}c@{}}31.5\\ 1.4\end{tabular} & \begin{tabular}[c]{@{}c@{}}4.9\\ 1.5\end{tabular} & \begin{tabular}[c]{@{}c@{}}12.0\\ 1.1\end{tabular} & \begin{tabular}[c]{@{}c@{}}14.6\\ 1.6\end{tabular} \\
PCS-JCT & \begin{tabular}[c]{@{}c@{}}avg JCT: 1.6\\ p99 JCT: 1.7\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.2\\ 1.4\end{tabular} & \begin{tabular}[c]{@{}c@{}}3.4\\ 4.5\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.0\\ 1.9\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.1\\ 1.1\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.6\\ 1.1\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.0\\ 1.2\end{tabular} \\
PCS-bal & \begin{tabular}[c]{@{}c@{}}avg JCT: 2.4\\ p99 JCT: 1.0\end{tabular} & \begin{tabular}[c]{@{}c@{}}3.4\\ 1.8\end{tabular} & \begin{tabular}[c]{@{}c@{}}3.2\\ 3.5\end{tabular} & \begin{tabular}[c]{@{}c@{}}5.4\\ 1.6\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.5\\ 1.3\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.5\\ 1.2\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.7\\ 1.0\end{tabular} \\
PCS-pred & \begin{tabular}[c]{@{}c@{}}avg JCT: 3.9\\ p99 JCT: 1.7\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.2\\ 1.4\end{tabular} & \begin{tabular}[c]{@{}c@{}}3.5\\ 4.5\end{tabular} & \begin{tabular}[c]{@{}c@{}}6.4\\ 1.4\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.6\\ 1.5\end{tabular} & \begin{tabular}[c]{@{}c@{}}4.3\\ 1.1\end{tabular} & \begin{tabular}[c]{@{}c@{}}6.0\\ 1.5\end{tabular} \\ \bottomrule
\end{tabular}%
}
\caption{JCT for traces}
\label{table:eval-trace-jct}
\end{table}

==> tables/table1-toy-example-case.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}


\begin{tabular}[b]{@{}cccc@{}}
\toprule
 & \begin{tabular}[c]{@{}c@{}}Arrival\\ Time\end{tabular} & \begin{tabular}[c]{@{}c@{}}Job\\ Size\end{tabular} & \begin{tabular}[c]{@{}c@{}}JCT\\ Fair\end{tabular} \\ \midrule
J1 & 0  & 10 & 24.5 \\
J2 & 0  & 8  & 20.5 \\
J3 & 1  & 1  & 3    \\
J4 & 10 & 8  & 17   \\ \bottomrule
\end{tabular}


==> tables/table2-toy-example-case.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

\begin{tabular}[b]{cccc}
\hline
 & \begin{tabular}[c]{@{}c@{}}Avg\\ JCT\end{tabular} & \begin{tabular}[c]{@{}c@{}}Max\\ Unfair\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg \\ \ecte{}\end{tabular} \\ \hline
Tiresias & \textbf{11.25} & 10\%  & 46\% \\
Themis   & 13.5  & \textbf{0\%}   & 24\% \\
YARN-FIFO     & 16.25 & 500\% & \textbf{0\%}  \\ \hline
% \vspace{0.5in}
\end{tabular}

